Learning based 2D Irregular Shape Packing

2D irregular shape packing is a necessary step to arrange UV patches of a 3D model within a texture atlas for memory-efficient appearance rendering in computer graphics. Being a joint, combinatorial decision-making problem involving all patch positions and orientations, this problem has well-known NP-hard complexity. Prior solutions either assume a heuristic packing order or modify the upstream mesh cut and UV mapping to simplify the problem, which either limits the packing ratio or incurs robustness or generality issues. Instead, we introduce a learning-assisted 2D irregular shape packing method that achieves a high packing quality with minimal requirements from the input. Our method iteratively selects and groups subsets of UV patches into near-rectangular super patches, essentially reducing the problem to bin-packing, based on which a joint optimization is employed to further improve the packing ratio. In order to efficiently deal with large problem instances with hundreds of patches, we train deep neural policies to predict nearly rectangular patch subsets and determine their relative poses, leading to linear time scaling with the number of patches. We demonstrate the effectiveness of our method on three datasets for UV packing, where our method achieves a higher packing ratio over several widely used baselines with competitive computational speed.

==> introduction.tex <==
\section{Introduction\label{sec:intro}}
2D irregular shape packing lies the theoretical foundation for a wide spectrum of applications across various industrial areas, e.g. material parts assembly~\cite{ke2020electric}, VLSI module placements~\cite{cheng2005floorplanning}, and 2D shelf arrangements in automatic warehouses~\cite{onut2008particle}. The most prominent packing application in computer graphics is UV chart packing, where a set of 2D shapes corresponding to patches of 3D models are packed together into a single texture atlas for mapping various appearance details onto the 3D surface for downstream rendering. In the realm of digital games where many 3D models are rendered in the virtual world, improving the UV packing ratio could significantly save the graphical memory, improve the loading speed, and reduce rendering overhead. This problem was recognized decades ago, e.g., by~\citet{soucy1996texture} and~\citet{sander2001texture}, which has recently revived as an active area of graphic research~\cite{limper2018box,Liu_AAAtlas_2019,zhang2020robust}.

Due to its combinatorial nature, finding optimal 2D shape packing has been well-understood as being NP-complete~\cite{hartmanis1982computers} and APX-hard~\cite{10.1287/moor.1050.0168}. The solution space for seeking the optimal solution is determined by the ordering of the to-be-packed patches, and the position and orientation of each patch. Prior research efforts are typically focusing on devising heuristic algorithms~\cite{10.3389/fmech.2022.966691} by first determining the packing order using simple heuristics or genetic algorithms~\cite{goodman1994genetic,liu2008solving} and then searching for the pose of each shape, e.g., using no-fit polygon (NFP)~\cite{bennell2008comprehensive} and the ``Tetris'' algorithm~\cite{levy2002least}. However, the sub-optimality gap of these heuristics can be substantial.
%
For applications having a loose computational time constraint, globally optimal stochastic optimization algorithms~\cite{goodman1994genetic,liu2008solving} have been proposed to search for the near-optimal packing orders. These techniques can scale to tens of 2D shapes, but UV unwrapping approaches~\cite{sorkine2002bounded,levy2002least,Dcharts2005} and commercial 3D modeling software~\cite{blender,UE5} can oftentimes generate hundreds of patches for one 3D model. In parallel, researchers have designed complex optimizations to restrict the UV charts during mesh cut and parameterization to be nearly rectangular, which in turn incurs robustness issues in practice~\cite{Liu_AAAtlas_2019}. %However, the aforementioned pipeline suffers from poor scalability due to the superlinear cost of computing the exact NFP via Minkowski sum, not to mention the globally optimal stochastic optimization algorithms~\cite{goodman1994genetic,liu2008solving}.

We propose a learning-assisted 2D packing pipeline for general irregular-shaped patches. The design of our approach is based on two observations: 1) High packing ratios can be achieved for nearly rectangular patches, as pointed out by~\cite{Liu_AAAtlas_2019}; 2) Tiny patches can be used to fill up void spaces between big patches. Accordingly, we split the input patches into tiny and non-tiny sets. Next, we iteratively group subsets of non-tiny patches into nearly rectangular super-patches. Our method's key challenge lies in identifying nearly rectangular patch subsets and the associated grouping strategy, for which we use a learning-assisted approach. We first leverage a high-level group selector network (HSN) to predict how likely a candidate patch subset can be grouped into a rectangular super-patch. Given an identified patch subset, we then use a low-level sorter network (LSN) to determine the suitable order of packing within the subset. Next, a low-level pose network (LPN) infers the rough initial pose of each patch. The ultimate pose of these patches is determined by local numerical optimization. After the super-patch is constructed, we insert it into the patch set for further grouping. The above process will be iterated until all the super-patches in the non-tiny set are nearly rectangular. Finally, we perform global assembly of the non-tiny super-patches using firstly bin-packing heuristics and then joint optimization to continuously adjust the patches for higher packing ratio, and we lastly use the scanline algorithm to fill the tiny patches into the gaps of non-tiny ones as our last step.

We have evaluated our method on 3 datasets, containing highly irregular UV patches generated from both organic and man-made 3D models. We show the effectiveness of our approach by comparing against widely used algorithm baselines, including piecewise linear NFP, XAtlas~\cite{Xatlas}, and~\cite{sander2003multi}, where we achieve a $5\%-10\%$ packing ratio improvement across all the tested datasets. We further highlight the generality of our learned policies, by training them on one dataset and evaluating them on all three datasets. We find our method still outperforming baselines on unseen datasets, proving that our method does not need to be retrained for each problem domain. We include the full datasets and results with statistics in the supplementary material.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> unused/figure.tex <==
%page 1: image
\begin{minipage}[c]{\textwidth}
\centering
%
\begin{minipage}{0.45\textwidth}
\begin{figure}[H]
\centering
%\frame{
\includegraphics[trim=0 0 1.2cm 1.2cm,clip,width=.99\linewidth]{fig/clocktime_v2.pdf}
%}
\vspace{-10px}
\caption{\label{fig:scalability}The average packing time of various algorithms plotted against the number of patches.}
\vspace{-5px}
\end{figure}
\end{minipage}
\hspace{0.05\textwidth}
%
\begin{minipage}{0.45\textwidth}
\begin{figure}[H]
\centering
\setlength{\tabcolsep}{1px}
\begin{tabular}{rrll}
\rotatebox{90}{\quad\quad After First Stage}&
\includegraphics[scale=.15]{fig/opt/pre_opt.png}&
\includegraphics[scale=.15]{fig/opt/after_opt.png}&
\rotatebox{90}{\quad\quad After Joint Opt.}\\
\rotatebox{90}{\;\TWORCell{No-filtering baseline}{pr: 71.9\%}}&
\includegraphics[scale=.15]{fig/fig3/withoutholefilling.png}&
\includegraphics[scale=.15]{fig/fig3/withholefilling.png}&
\rotatebox{90}{\quad\TWORCell{After Hole-filling}{pr: 76.5\%}}\\
%& pr: 71.9\% & pr: 76.5\% &
\end{tabular}
\vspace{-5px}
\caption{\label{fig:stageTwo} After the first stage, there are gaps between non-tiny patches (top left). We perform a joint optimization to squeeze patches and remove gaps (top right). After hole-filing, we achieve a packing ratio of $76.5\%$ (bottom right). If we do not filter out the tiny patches and forward all patches to HSN, we can only achieve a ratio of $71.9\%$ (bottom left).}
\vspace{-5px}
\end{figure}
\end{minipage}
%
\begin{minipage}{\textwidth}
\begin{figure}[H]
\centering
\bgroup
\def\arraystretch{.5}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccc}
\toprule
 & \scalebox{0.7}{\cite{sander2003multi}} & \scalebox{0.7}{XAtlas} & \scalebox{0.7}{NFP} & \scalebox{0.7}{Ours}\\
 \midrule
\includegraphics[scale=.1]{fig/fig4/house_model.png}&
\includegraphics[scale=.1]{fig/fig4/house_2003_0.695.png}&
\includegraphics[scale=.1]{fig/fig4/house_xatlas_0.701.png}&
\includegraphics[scale=.1]{fig/fig4/house_nfp_0.745.png}&
\includegraphics[scale=.1]{fig/fig4/house_ours_0.824.png}\\
 & \scalebox{0.7}{pr: 69.5\%} &\scalebox{0.7}{pr: 70.1\%} & \scalebox{0.7}{pr: 74.5\%} & \scalebox{0.7}{pr: 82.4\%}\\
 \midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\includegraphics[scale=.1]{fig/fig4/cat_model.png}&
\includegraphics[scale=.1]{fig/fig4/cat_2003_0.689.png}&
\includegraphics[scale=.1]{fig/fig4/cat_xatlas_0.654.png}&
\includegraphics[scale=.1]{fig/fig4/cat_nfp_0.647.png}&
\includegraphics[scale=.1]{fig/fig4/cat_ours_0.772.png}\\
 & \scalebox{0.7}{pr: 68.9\%} &\scalebox{0.7}{pr: 65.4\%} & \scalebox{0.7}{pr: 64.7\%} & \scalebox{0.7}{pr: 77.2\%}\\
 \midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\includegraphics[scale=.1]{fig/fig4/ramses_model.png}&
\includegraphics[scale=.1]{fig/fig4/ramses_2003_0.670.png}&
\includegraphics[scale=.1]{fig/fig4/ramses_xatlas_0.679.png}&
\includegraphics[scale=.1]{fig/fig4/ramses_nfp_0.690.png}&
\includegraphics[scale=.1]{fig/fig4/ramses_ours_0.7680.png}\\
 & \scalebox{0.7}{pr: 67.0\%} &\scalebox{0.7}{pr: 67.9\%} & \scalebox{0.7}{pr: 69.0\%} & \scalebox{0.7}{pr: 76.8\%}\\
 \bottomrule
\end{tabular}}
\egroup
\vspace{-5px}
\caption{\label{fig:result_of_dataset}Three packing instances from the building, organic and general dataset.}
\vspace{-5px}
\end{figure}
\end{minipage}
\end{minipage}


%page 2: image
\begin{figure*}[ht]
\centering
\bgroup
\def\arraystretch{.5}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c}
\scalebox{0.5}{Building} & \scalebox{0.5}{Organic} & \scalebox{0.5}{General}\\
\includegraphics[scale=.1]{fig/dataset/dataset_building.png}&
\includegraphics[scale=.1]{fig/dataset/dataset_organic.png}&
\includegraphics[scale=.1]{fig/dataset/dataset_general.png}\\
\end{tabular}}
\egroup
\vspace{-5px}
\caption{\label{fig:dataset}A set of 3D model samples from our three datasets.}
\vspace{-5px}
\end{figure*}
%
\begin{figure*}[ht]
\centering
\bgroup
\def\arraystretch{.5}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccc}
\toprule
 & \scalebox{0.7}{\cite{sander2003multi}} & \scalebox{0.7}{XAtlas} & \scalebox{0.7}{NFP} & \scalebox{0.7}{Ours}\\
 \midrule
\includegraphics[scale=.1]{fig/fig5/animalchess_model.png}&
\includegraphics[scale=.1]{fig/fig5/animalchess_2003_0.596.png}&
\includegraphics[scale=.1]{fig/fig5/animalchess_xatlas_0.674.png}&
\includegraphics[scale=.1]{fig/fig5/animalchess_nfp_0.723.png}&
\includegraphics[scale=.1]{fig/fig5/animalchess_ours_0.759.png}\\
 & \scalebox{0.7}{pr: 59.6\%} &\scalebox{0.7}{pr: 67.4\%} & \scalebox{0.7}{pr: 72.3\%} & \scalebox{0.7}{pr: 75.9\%}\\
\bottomrule
\end{tabular}}
\egroup
\vspace{-10px}
\caption{\label{fig:large_example}A large problem instance with $784$ charts.}
\vspace{-5px}
\end{figure*}
%
\begin{figure*}[ht]
\centering
\bgroup
\def\arraystretch{.5}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccc}
\toprule
 & \scalebox{0.7}{\cite{sander2003multi}} & \scalebox{0.7}{XAtlas} & \scalebox{0.7}{NFP} & \scalebox{0.7}{Ours}\\
 \midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \includegraphics[scale=.1]{fig/fig7/building4_model.png}&
\includegraphics[scale=.1]{fig/fig7/building4_2003_0.592.png}&
\includegraphics[scale=.1]{fig/fig7/building4_xatlas_0.664.png}&
\includegraphics[scale=.1]{fig/fig7/building4_nfp_0.530.png}&
\includegraphics[scale=.1]{fig/fig7/building4_ours_0.737.png}\\
 & \scalebox{0.7}{pr: 59.2\%} &\scalebox{0.7}{pr: 66.4\%} & \scalebox{0.7}{pr: 53.0\%} & \scalebox{0.7}{pr: 73.7\%}\\
 \midrule
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\includegraphics[scale=.1]{fig/fig7/max_model.png}&
\includegraphics[scale=.1]{fig/fig7/max_2003_0.669.png}&
\includegraphics[scale=.1]{fig/fig7/max_xatlas_0.639.png}&
\includegraphics[scale=.1]{fig/fig7/max_nfp_0.592.png}&
\includegraphics[scale=.1]{fig/fig7/max_ours_0.746.png}\\
 & \scalebox{0.7}{pr: 66.9\%} &\scalebox{0.7}{pr: 63.9\%} & \scalebox{0.7}{pr: 59.2\%} & \scalebox{0.7}{pr: 74.6\%}\\
 \midrule
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\includegraphics[scale=.1]{fig/fig7/wizard_model.png}&
\includegraphics[scale=.1]{fig/fig7/wizard_2003_0.548.png}&
\includegraphics[scale=.1]{fig/fig7/wizard_xatlas_0.542.png}&
\includegraphics[scale=.1]{fig/fig7/wizard_nfp_0.555.png}&
\includegraphics[scale=.1]{fig/fig7/wizard_ours_0.621.png}\\
 & \scalebox{0.7}{pr: 54.8\%} &\scalebox{0.7}{pr: 54.2\%} & \scalebox{0.7}{pr: 55.5\%} & \scalebox{0.7}{pr: 62.1\%}\\
\bottomrule
\end{tabular}}
\egroup
\vspace{-10px}
\caption{\label{fig:more_results_2}Three packing instances from the building, organic, and general dataset.}
\vspace{-5px}
\end{figure*}

==> xr.tex <==
%----Helper code for dealing with external references----
% (by cyberSingularity at http://tex.stackexchange.com/a/69832/226)

\usepackage{xr}
\makeatletter

\newcommand*{\addFileDependency}[1]{% argument=file name and extension
\typeout{(#1)}% latexmk will find this if $recorder=0
% however, in that case, it will ignore #1 if it is a .aux or 
% .pdf file etc and it exists! If it doesn't exist, it will appear 
% in the list of dependents regardless)
%
% Write the following if you want it to appear in \listfiles 
% --- although not really necessary and latexmk doesn't use this
%
\@addtofilelist{#1}
%
% latexmk will find this message if #1 doesn't exist (yet)
\IfFileExists{#1}{}{\typeout{No file #1.}}
}\makeatother

\newcommand*{\myexternaldocument}[1]{%
\externaldocument{#1}%
\addFileDependency{#1.tex}%
\addFileDependency{#1.aux}%
}
%------------End of helper code--------------
